TALUS: Reinforcing TEE Confidentiality with Cryptographic Coprocessors (Technical Report)

Platforms are nowadays typically equipped with tristed execution environments (TEES), such as Intel SGX and ARM TrustZone. However, recent microarchitectural attacks on TEEs repeatedly broke their confidentiality guarantees, including the leakage of long-term cryptographic secrets. These systems are typically also equipped with a cryptographic coprocessor, such as a TPM or Google Titan. These coprocessors offer a unique set of security features focused on safeguarding cryptographic secrets. Still, despite their simultaneous availability, the integration between these technologies is practically nonexistent, which prevents them from benefitting from each other's strengths. In this paper, we propose TALUS, a general design and a set of three main requirements for a secure symbiosis between TEEs and cryptographic coprocessors. We implement a proof-of-concept of TALUS based on Intel SGX and a hardware TPM. We show that with TALUS, the long-term secrets used in the SGX life cycle can be moved to the TPM. We demonstrate that our design is robust even in the presence of transient execution attacks, preventing an entire class of attacks due to the reduced attack surface on the shared hardware.

==> chapters/changelog.tex <==
%!TEX root=../main.tex


In this section, we summarize the changes for our revised version of the paper. All the changes and additions are highlighted for ease of identification and annotated with the relevant questions from the accompanying rebuttal text.

\subsection{Extended Systematization}

Due to page restriction, we originally removed a big portion of the systematization in \Cref{ReAnalSystematization} from the submitted version of the paper. The revised version now details the comparison between the trusted computing candidates we have introduced in \Cref{ReAnalSystematization} in regards to the features \emph{strict hardware isolation} and \emph{confidentiality and integrity of storage} for \emph{Security Properties}, and \emph{untrusted software dependencies} and \emph{secure counter} for \emph{Secure Storage}. %In this revision we tried to present in a compact form in \Cref{ReAnalSystematization} under the head \emph{Security Properties (SP)} and \emph{Secure Storage (SC)}.
The new \Cref{tab:systematizationObjectives} summarizes the new text.
This additional comparison highlights in particular the shortcomings of TEEs alone and how/which coprocessors can fill this gap when securely integrated according to our requirements from \Cref{tab:systematizationRequirements}.
We believe the revised and extended systematization of different TEEs and coprocessors will help to better understand the motivation for our solution and answer some of the comments raised by the reviewers.


\subsection{TALUS versus Improved SGX}

% Removed: this is a changelog and not a rebuttal text
% The extended systematization depicts that SGX lacks trusted replay-protected storage (\Cref{tab:systematizationObjectives}). Even after numerous fixes and updates, \sgx is forced to use the memory hierarchy as local staging buffer for cryptographic secrets, where other untrusted softwares are running in parallel. This unavailability of storage does not allow \sgx to store and maintain a trusted counter that could have identified how often the enclave is interrupted and could have given the developer or system a chance to decide to restart after a developer/system-defined number. The improved \sgx also falls victim to the current architecture not supporting replay-protected storage owned by the processor. The Intel PTT offers a temporary BIOS SPI storage. But upon a system restart or BIOS battery removal this storage can be reset (\Cref{ReAnalSystematization} Secure Storage (SSC)). So we believe as long as a confidentiality- and integrity-protected tamper-resistant storage is not introduced to SGX it is not possible to improve SGX by simply updating the firmware. TALUS is doing exactly that by introducing TPM to SGX's life-cycle.

We rephrased the paragraph \emph{TALUS: Intel SGX and Hardware TPM} in \Cref{ReAnalSystematization} to summarize our beliefs why an improved SGX cannot provide the same security benefits as SGX with the \emph{hardware} TPM as integrated coprocessor.
Those beliefs are also rooted in the results from our extended systematization.

The extended systematization depicts that SGX lacks trusted replay-protected storage (\Cref{tab:systematizationObjectives}).
Even after numerous fixes and updates, \sgx is forced to use the memory hierarchy as local staging buffer for cryptographic secrets, where other untrusted software is running in parallel.
This unavailability of storage does not allow \sgx to store and maintain a trusted counter that could have identified how often the enclave is interrupted and could have given the developer or system a chance to decide to restart after a developer/system-defined number.
An improved \sgx that relies only on firmware changes also falls victim to the current architecture not supporting replay-protected storage owned by the processor.
The extended systematization shows that Intel PTT offers a temporary BIOS SPI storage that can be reset upon a system restart or BIOS battery removal.
So we believe it is not possible to improve SGX by simply updating the firmware as long as a confidentiality- and integrity-protected tamper-resistant storage is not introduced to SGX.
TALUS is doing exactly that by integrating \emph{hardware} TPM (and its NVM) within SGX.

\subsection{Porting to other platforms}

We have extended \Cref{otherplatfrom} about how TALUS can be ported to other platforms (e.g., ARM, RISC V).
While each platform requires its own engineering effort to implement our requirements from \Cref{tab:systematizationRequirements}, our proof-of-concept prototype with TPM and SGX provides valuable lessons learned.
We provided those insights in the revised version when comparing our building blocks (like measured code in SGX and locality from SMM/TXT) to those available (and missing) in other TEEs and coprocessors (like NS-bit in ARM TZ or register-based communication in RoCC).



% The NS bit can help the processor differentiate calls between Android and Trustzone, ensuring vertical access control. Nonetheless, ARM platforms for both Android and Apple do not provide support for secure communication channels or horizontal access control.

% The case is same for RISC-V. We have explained how RoCC accelerator offers a TALUS-type register-based communication channel. But does not support vertical access control or horizontal access control.

% We believe that exporting TALUS to ARM or RISC-V is mostly a technical implementation.
% The design of TALUS can heavily improve both ARM and RISC-V platforms.

\subsection{Security guarantees regarding replay attack protection}

We like to apologize for the misunderstanding between replay attacks and attacks that can be prevented by using replay-protected storage.
We have updated the summary section in the Introduction about how TALUS leverages TPM’s NVM to store trusted and persistent counters that can be used by SGX to limit precise execution control attacks against enclaves.
We have explained this countermeasure in Section~6.2 (text not changed from original submission).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:


==> chapters/discussionV2.tex <==
%!TEX root=../main.tex

\noted{discuss integration possibilities on other platform. Atleast ARM and RISCV. this paper is x86}

Various coprocessors and TEEs and their combined implementations running on the application processor offer very similar use-cases (\eg containerized code execution, confidentiality and integrity of the container, or attestation). 
As they are bound to use the underlying architecture, they often inherit vulnerabilities of the platform. 
Since the discovery of microarchitectural and side-channel attacks, not only code or data that TEEs working on are jeopardized but also their infrastructure secrets are compromised.  
At this point, we systematically (\cf \Cref{objDefinition}) documented a list of objectives that we believe these combinations should deliver to preserve confidentiality and integrity.
Comparing some industrial and research TEE-Coprocessor combinations against those objectives (for the first time), our understanding improves with their shortcomings. 
We pin-point the gaps and identified that there is a demand of an example TEE-Coprocessor implementation achieving all the objectives we deviced. 
Hence we implemented \ourname, a prototype, showing how to achieve all the objectives keeping the underlying hardware infrastructure unchanged. 
All the changes that we introduced for our prototype are readily patchable through firmware and microcode updates.
However, \ourname is not limited to SGX but also applies to other TEEs, \eg  Intel-SGX, AMD SEV, ARM TrustZone or RISC-V Keystone. % as they work in a similar fashion utilizing the same underlying hardware infrastructure.
 
While designing \ournameplain, we keep in mind that the coprocessor's usecases are not limited to TEE but also supporting other clients on the platform (\eg a software needs a \tpm generated key). 
We use the \tpm locality to identify from which security ring the client is requesting from (vertical access control) and \tpm EAP to differentiate client within a security ring, although Locality and EAP is integrated with \sgx also.  

By design, \sgx enclaves cannot access peripheral hardware. 
In \ourname, we provide enclaves controlled access to the \tpm. 
Related work also provided \sgx with direct access to the GPU~\cite{Insu2019}, or generic I/O devices~\cite{Weiser2017sgxio}. 
For other peripherals without such existing support, solutions like DICE/RIOT~\cite{england2016riot,england2017device,TCGDice} could be a way forward to securely integrate them with SGX or other TEEs.


\ourname depends on pre-shared keys between CPU and TPM. 
While this might seem cumbersome, it is in line with existing designs.
SGX, PSP or Titan, all uses pre-shared secrets.
A pre-shared key between CPU and TPM enables command parameter encryption to safeguard the communication channel and to create a strong cryptographically provable binding between the CPU and the TPM. 
Otherwise, as shown by the Dolos attack~\cite{dolosattack}, missing TPM parameter encryption enables attackers to access disk encryption keys in the TPM. 
Establishing trust without a pre-shared key pair is difficult, as proving trust on the go is still an open problem, and thus out of the scope for this paper.

Close to \ourname is Intel PTT which includes a firmware \tpm, compliant to Microsoft's fTPM~\cite{Raj2016} running inside Intel CSME~\cite{Cen2017}. 
However, PTT fall short to provide enough security due to Intel CSME's vulnerabilities (see \Cref{objPTT}) (some of them are unpatchable) and encourages us to dig deeper into the problem and possibly to find an alternative solution which is also easy to deploy. 

Another research article closer to \ournameplain is a poster by Chakra-borty~\etal\cite{chakraborty2018NDSS}.
The authors propose using a \tpm for securing the secrets for enclave building and launch. 
However, they did not consider any of the challenges for integrating the \tpm with \sgx. 
In our work, we fill the gap and demonstrate an actual design for integrating a coprocessor with a secure enclave.  
We evaluate our prototype using \tpm and \sgx against our objectives, and present additional use cases for impeding microarchitectural attacks. 

We focus on desktop and server CPUs. 
For low-end embedded devices, \textit{VRASED}~\cite{Nunes2019} and \textit{APEX}~\cite{nunes2019verified} showed how a coprocessor that monitors execution signals on the main processor can provide verified attestation and proofs-of-execution of pieces of code. 
Transferring our idea, one could investigate how such pieces of code could have exclusive access to secrets via the coprocessor.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:


==> chapters/evaluation.tex <==
%!TEX root=../samplepaper.tex

%\begin{figure}[t]
%	\centering
%%         \includegraphics[width=\linewidth]{figures/measurements32_1}
%    \input{figures/performance.tikz}
%	\caption{Performance of different SGX commands for \ournameplain with \tpm (average time and standard error).}
%	\label{fig:measurements_paper}
%\end{figure}
%%
%\begin{figure}[t]
%	\centering
%% 	\includegraphics[width=\linewidth]{figures/buildmeasurements1}
%    \input{figures/performance-sgx.tikz}
%	\caption{Performance comparison (in \textit{ms}): enclave management of \sgx against \ournameplain. }
%	\label{fig:measurements_highlevel_paper}
%\end{figure}


%\begin{figure}%
%	\centering
%	\subfloat[\tpm Performance of different SGX commands for \ournameplain with \tpm (average time and standard error).]{{\input{figures/performance.tikz} }}%
%	\qquad
%	\subfloat[Performance comparison (in \textit{ms}): enclave management of \sgx against \ournameplain.]{{\input{figures/performance-sgx.tikz} }}%
%	\caption{2 \ournameplain performance evaluation}%
%	\label{fig:measurements_paper}%
%\end{figure}

% \begin{table}[t]
% 	\centering
% 	\footnotesize
% 	\begin{tabular}{|r || c | c |}
% 		\hline
% 		& \textbf{Host} & \textbf{Guest}  \\
% 		\hline
% 		\hline
% 		\textbf{OS} & Ubuntu 16.04.4 64bit & Ubuntu 16.04.4 64bit \\
% 		\textbf{Kernel} & 5.0.0+ & 5.0.0+ \\
% 		\textbf{CPU} & Intel i7-6700 & Intel i7-6700 \\
% 		\textbf{SGX} & KVM-SGX, QEMU-SGX & SGX SDK 2.0 \\
% 		\hline
% 	\end{tabular}
% 	\caption{Prototype system configurations}
% 	\label{table:prototype}
% \end{table}

%\input{chapters/evaluationResultTable}
%In this section, we evaluate the performance of \ourname. 
%As there is no publicly-available cycle-accurate CPU emulator with SGX support, we can only provide bounds for the performance of \ourname. 
%Thus, the evaluation consists of two parts. 
%In the first part, we run the SGX enclaves inside KVM with SGX support~\cite{intelVirtSGX,kvmSGX} using QEMU-KVM~\cite{qemuSGX} to implement the protected communication channel (\cf \Cref{harpocrates}) in the hypervisor. 
%In the second part, to judge the overhead of the hypervisor, we evaluate native enclaves, but without the protection of the communication channel. 
%All evaluations are done on an Intel i7-7820X running Ubuntu 16.04.04 with kernel 5.0.0.
%As a TPM, we use an Infineon SLB 9670 supporting TPM 2.0 (HTPM), and a software \tpm%\notem{sw-TPM? Software TPM? STPM? fTP? unify the terms!} 
%from IBM~\cite{softTPM}. The size of the enclave used for performance evaluation is 52 KB.

% We believe \textit{qemuSTPM} is the closest setup to an SGX supported by Intel-PTT. 

%\subsection{Primitives}
%We evaluate the runtime of the primitives provided by \ourname. 
%All primitives are used in a secure end-to-end communication between an SGX enclave and the TPM. 
%As a baseline, we measure the time it takes the hardware TPM to execute these primitives. 
%Figure~\ref{fig:measurements_paper}.a shows the timing for the baseline (HTPM) and the variants of our proof-of-concept implementation using the hardware (QEMU HTPM) and software (QEMU STPM) TPM. 
%We repeat all measurements 1,000 times and present the average and a \SI{95}{\percent} confidence interval.
%Depending on the primitive, the communication between the TPM and SGX adds an average overhead between \SI{0.49}{\milli\second} (generating a 2048-bit RSA key) and \SI{50.77}{\milli\second} (enclave signing). 
%This shows that \ourname itself does not add a significant overhead. 
%Unsurprisingly, the software TPM outperforms the hardware TPM in all scenarios.
%As a result, the software-backed \ourname performs significantly better (factor 2 to 38) than the hardware-backed \ourname. 
%
%\ournameplain running with a hardware \tpm adds an average overhead of \SI{98.61}{\milli\second}$\pm$\SI{1.95}{\milli\second}. 
%\ournameplain with software \tpm adds an average overhead of \SI{5.62}{\milli\second}$\pm$\SI{0.17}{\milli\second}, whereas a hardware \tpm generally adds \SI{76.05}{\milli\second}$\pm$\SI{1.42}{\milli\second} of overhead for similar types of commands. 
%Note that the overall runtime overhead of an enclave depends on its workload, \ie how often these commands are executed. 

%\subsection{\ournameplain-backed Enclave Handling}
%For macro benchmarking, we evaluate the performance of our first case study, the \ourname-backed enclave management described in \Cref{UC:tpmbasedenclavebuilding}. 
%Figure~\ref{fig:measurements_paper}.b shows the performance of the TPM-backed functions required to create and launch an SGX enclave. 
%The enclave creation, which includes allocating enclave pages, measuring page contents, and verifying the measurements, takes on average \SI{624.16}{\milli\second} with \ourname and a hardware TPM (QEMU-HTPM). 
%Compared to vanilla SGX, which also takes \SI{97.75}{\milli\second}, this is only an overhead of \SI{526.41}{\milli\second}.
%Given that the creation of an enclave is a one-time event in the life cycle of an enclave and does not affect any operation at runtime, this overhead is likely amortized over the runtime of the enclave. 
%Again, when backed by a software TPM, the overhead is much smaller with only \SI{144.07}{\milli\second}. 
%Similarly, the enclave launch takes, on average, \SI{477.23}{\milli\second} longer than in vanilla SGX. 
%With a software TPM, our \ourname proof-of-concept is nearly as fast as vanilla SGX, with an overhead of only \SI{7.75}{\milli\second}. 

\subsection{Data Encryption}
We evaluate a real-world use case that encrypts data using AES without leaking any key material to an attacker, even in the presence of transient execution attacks, hyperthreading, and precise execution control (\cf \Cref{UC:mitigations}).
Our application uses a 128-bit AES key securely stored in the TPM, only fetched when encrypting user-provided data. 
To ensure no leakage of round keys via the SSA, we execute the round-key derivation and encryption within a hardware transaction. 
The total runtime of encrypting \SI{4}{\kilo B} of data and cleaning up any secret state is \SI{1.66}{\micro\second}$\pm$\SI{0.001}{\micro\second}, excluding fetching the key from the TPM.
The overhead from \ourname, \ie securely getting the key, is \SI{58.43}{\milli\second}$\pm$\SI{1.45}{\milli\second}. 
As a baseline, we compare the runtime to a variant where the key is not fetched from the TPM but is instead unsealed from the disk. 
This (insecure) variant has an average runtime of \SI{199.21}{\micro\second}$\pm$\SI{0.45}{\micro\second}.
Note that the one-time overhead is amortized if the enclave runtime increases, \eg if larger amounts of data are encrypted. 


\subsection{CPU-integrated \ournameplain Performance}

%\begin{figure}[t]
%\centering
%\resizebox{\hsize}{!}{
% \input{figures/overhead.tikz}
% }
% \caption{The total runtime of the commands split into base execution time and the overhead added by QEMU. }
% \label{fig:qemu-overhead}
%\end{figure}


Since only Intel can implement a native version of \ourname, and there is no cycle-accurate emulator supporting SGX, we can only provide an estimation for such a version. 
\Cref{fig:qemu-overhead} shows the overhead added by QEMU for the \ourname commands, adding an overhead between \SIrange{5}{10}{\milli\second} (avg. of \SI{6.82}{\milli\second}). 
% For \textit{qemuSTPM}, this overhead constitutes between 38.79\% to almost 100\% of the end-to-end runtime, depending on the command, with an average of 51.77\%. In contrast, for \htpm between 4.37\%--63.71\% (average 34.04\%). 
This overhead constitutes between \SIrange{2.21}{38.77}{\percent} (avg. of \SI{21.60}{\percent}). 
We assume that the native \ourname performance ise around \SI{20}{\percent} faster on average for each command. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:


==> chapters/evaluationResultTable.tex <==
%!TEX root=../bare_conf.tex

\begin{table}[h]
	\caption{Performance comparison (in ms) of different SGX commands for \ournameplain with TPM (see \Cref{fig:measurements_paper}).}
	\label{tab:perfcompcommand}

	\begin{tabular}{ccrrrr}
		\toprule
        \small \tikz \node[rotate=0] {\textbf{\scriptsize Test}}; & 
		\small \tikz \node[rotate=0] {\textbf{\scriptsize Device}}; &  
		\multicolumn{1}{c}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Max}}};} & 
		\multicolumn{1}{c}{\small \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Min}}};} &  
		\multicolumn{1}{c}{\small \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Mean $\pm$ CI}}};} & 
		\multicolumn{1}{c}{\small \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Median}}};} \\
		%\small \tikz \node[rotate=90] {\textbf{\shortstack{Confidence \\ interval}}}; \\
		\midrule
		\multirow{3}{*}{\footnotesize get key} & 
		\footnotesize{HTPM} & 
		\footnotesize 600 & 
		\footnotesize 200 & 
		\footnotesize 400.46 $\pm$ 7.07 & 
		\footnotesize 398 \\
		& \footnotesize{qemuHTPM} & 
		\footnotesize 652 & 
		\footnotesize 156 & 
		\footnotesize 400.96 $\pm$ 8.97 & 
		\footnotesize 397 \\
		& \footnotesize{qemuSTPM} & 
		\footnotesize 20 & 
		\footnotesize 1 & 
		\footnotesize 10.57 $\pm$ 0.34 & 
		\footnotesize 11 \\
		\midrule
		\multirow{3}{1cm}{\footnotesize get counter} & 
		\footnotesize{HTPM} & 
		\footnotesize 10 & 
		\footnotesize 5 & 
		\footnotesize 7.48 $\pm$ 0.09 & 
		\footnotesize 7 \\
		\footnotesize & 
		\footnotesize{qemuHTPM} & 
		\footnotesize 13 & 
		\footnotesize 5 & 
		\footnotesize 8.95 $\pm$ 0.14 & 
		\footnotesize 9 \\
		 & \footnotesize{qemuSTPM} & \footnotesize 6 & \footnotesize 2 & \footnotesize 3.96 $\pm$ 0.08 & \footnotesize 4 \\
		\midrule
		\multirow{3}{1cm}{\footnotesize get time}& \footnotesize{HTPM} & \footnotesize 17 & \footnotesize 5 & \footnotesize 11.13 $\pm$ 0.22 & \footnotesize 11 \\
		\footnotesize & \footnotesize{qemuHTPM} & \footnotesize 52 & \footnotesize 20 & \footnotesize 36.38 $\pm$ 0.58 & \footnotesize 37 \\
	    & \footnotesize{qemuSTPM} & \footnotesize 24 & \footnotesize 2 & \footnotesize 6.06 $\pm$ 0.20 & \footnotesize 6  \\
	    \midrule
	    \multirow{3}{1cm}{\footnotesize load key} & \footnotesize{HTPM} & \footnotesize 17 & \footnotesize 3 & \footnotesize 9.92 $\pm$ 0.25 & \footnotesize 10 \\
	    \footnotesize & \footnotesize{qemuHTPM} & \footnotesize 42 & \footnotesize 17 & \footnotesize 29.72 $\pm$ 0.45 & \footnotesize 30 \\
	    & \footnotesize{qemuSTPM} & \footnotesize 14 & \footnotesize 2 & \footnotesize 4.45 $\pm$ 0.16 & \footnotesize 5  \\
	    \midrule
	    \multirow{3}{1cm}{\footnotesize quote} & \footnotesize{HTPM} & \footnotesize 17 & \footnotesize 3 & \footnotesize 9.92 $\pm$ 0.25 & \footnotesize 10 \\
	    & \footnotesize{qemuHTPM} & \footnotesize 65 & \footnotesize 30 & \footnotesize 47.47 $\pm$ 0.63 & \footnotesize 47 \\
	    & \footnotesize{qemuSTPM} & \footnotesize 19 & \footnotesize 1 & \footnotesize 3.75 $\pm$ 0.09 & \footnotesize 4  \\
	    \midrule
	    \multirow{3}{1cm}{\footnotesize sign enclave} & \footnotesize{HTPM} & \footnotesize 35 & \footnotesize 1 & \footnotesize 17.40 $\pm$ 0.64 & \footnotesize 17 \\
	    \footnotesize  & \footnotesize{qemuHTPM} & \footnotesize 95 & \footnotesize 41 & \footnotesize 68.14 $\pm$ 0.98 & \footnotesize 68 \\
	    & \footnotesize{qemuSTPM} & \footnotesize 15 & \footnotesize 2 & \footnotesize 4.91 $\pm$ 0.16 & \footnotesize 5 \\
	    \bottomrule
	\end{tabular}
\end{table}

\begin{table}[h]
	\caption{Performance comparison (in ms): enclave management of \sgx against \ournameplain (see \Cref{fig:measurements_highlevel_paper}).}
	\label{tab:perfcommsgxfunction}
	
	\begin{tabular}{ccrrrr}
		\toprule
		\small \tikz \node[rotate=0] {\textbf{\scriptsize Test}}; & 
		\small \tikz \node[rotate=0] {\textbf{\scriptsize Device}}; &  
		\multicolumn{1}{c}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Max}}};} & 
		\multicolumn{1}{c}{\small \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Min}}};} &  
		\small \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Mean $\pm$ CI}}}; & 
		%\small \tikz \node[rotate=90] {\textbf{\shortstack{Median \\ (in ms)}}}; &
		\multicolumn{1}{c}{\small \tikz \node[rotate=0] {\textbf{\shortstack{\scriptsize Median}}};} \\
		\midrule
		\multirow{3}{1cm}{\footnotesize{Enclave Building}} & \footnotesize{vanilla SGX} & \footnotesize 180 & \footnotesize 14 & \footnotesize 97.75 $\pm$ \phantom{0}2.98  & \footnotesize 98 \\
		 & \footnotesize{qemuHTPM} & \footnotesize 823 & \footnotesize 436 & \footnotesize 624.16 $\pm$ \phantom{0}6.83 & \footnotesize 623  \\
		\footnotesize & \footnotesize{qemuSTPM} & \footnotesize 422 & \footnotesize 50 & \footnotesize 241.82 $\pm$ \phantom{0}6.78 & \footnotesize 245  \\
		\midrule
		\multirow{3}{1cm}{\footnotesize{Enclave Launch}} & \footnotesize{vanilla SGX} & \footnotesize 45 & \footnotesize 9 & \footnotesize 26.83 $\pm$ \phantom{0}0.64 & \footnotesize 27  \\
		& \footnotesize{qemuHTPM} & \footnotesize 800 & \footnotesize 230 & \footnotesize 504.06 $\pm$ 10.40 & \footnotesize 504  \\
		& \footnotesize{qemuSTPM} & \footnotesize 58 & \footnotesize 12 & \footnotesize 34.58 $\pm$ \phantom{0}0.81 & \footnotesize 34 \\
		\bottomrule
	\end{tabular}

\end{table}

%\begin{table*}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		\multirow{2.3}{*}\small \tikz \node[rotate=90] {\textbf{\shortstack{}}}; & 
%	    %\multicolumn{3}{c|}{\small  \tikz \node[rotate=90] {\textbf{\shortstack{enclaveBuild}}};} &
%	    %\multicolumn{3}{c|}{\small  \tikz \node[rotate=90] {\textbf{\shortstack{enclaveLaunch}}};} &
%	    \multicolumn{3}{c|}{\footnotesize  \tikz \node[rotate=0] {\textbf{\shortstack{get\_Key}}};} &
%	    \multicolumn{3}{c|}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{read\_counter}}};} &
%	    \multicolumn{3}{c|}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{get\_time}}};} &
%	    \multicolumn{3}{c|}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{load\_key}}};} &
%	    \multicolumn{3}{c|}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{quote}}};} &
%	    \multicolumn{3}{c|}{\small  \tikz \node[rotate=0] {\textbf{\shortstack{sign\_Enckave}}};} \\
%	    \cline{2-19}
%	    \small  \tikz \node[rotate=90] {\textbf{\shortstack{Measurements}}}; &
%		\small  \tikz \node[rotate=90] {\textbf{\shortstack{HTPM}}}; & 
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuHTPM}}}; &  
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuSTPM}}}; & 
%		\small  \tikz \node[rotate=90] {\textbf{\shortstack{HTPM}}}; & 
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuHTPM}}}; &  
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuSTPM}}}; &  
%		\small  \tikz \node[rotate=90] {\textbf{\shortstack{HTPM}}}; & 
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuHTPM}}}; &  
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuSTPM}}}; &
%		\small  \tikz \node[rotate=90] {\textbf{\shortstack{HTPM}}}; & 
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuHTPM}}}; &  
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuSTPM}}}; &
%		\small  \tikz \node[rotate=90] {\textbf{\shortstack{HTPM}}}; & 
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuHTPM}}}; &  
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuSTPM}}}; &
%		\small  \tikz \node[rotate=90] {\textbf{\shortstack{HTPM}}}; & 
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuHTPM}}}; &  
%		\small \tikz \node[rotate=90] {\textbf{\shortstack{qemuSTPM}}}; \\
%		\hline \hline
%		\small{\shortstack{Maximum \\ (in ms)}} & 
%		\small 600 & \small 652 & \small 20 & 
%		\small 10 & \small 13 & \small 6 & 
%		\small 17 & \small 52 & \small 24 & 
%		\small 17 & \small 42 & \small 14 & 
%		\small 17 & \small 65 & \small 19 & 
%		\small 35 & \small 95 & \small 15 \\
%		\hline
%		
%		\small{\shortstack{Minimum \\ (in ms)}} & 
%		\small 200 & \small 156 & \small 1 & 
%		\small 5 & \small 5 & \small 2 & 
%		\small 5 & \small 20 & \small 1 & 
%		\small 3 & \small 17 & \small 0 & 
%		\small 3 & \small 30 & \small 1 & 
%		\small 1 & \small 41 & \small 1 \\
%		\hline
%		
%		\small{\shortstack{Mean \\ (in ms)}} & 
%		\small 400.46 & \small 400.96 & \small 10.57 & 
%		\small 7.48 & \small 8.95 & \small 3.96 & 
%		\small 11.13 & \small 36.38 & \small 6.06 & 
%		\small 9.92 & \small 29.72 & \small 4.45 & 
%		\small 9.92 & \small 47.47 & \small 3.75 & 
%		\small 17.40 & \small 68.14 & \small 4.91 \\
%		\hline
%		
%		\small{\shortstack{Median \\ (in ms)}} & 
%		\small 398 & \small 397 & \small 11 & 
%		\small 7 & \small 9 & \small 4 & 
%		\small 11 & \small 37 & \small 6 & 
%		\small 10 & \small 30 & \small 5 & 
%		\small 10 & \small 47 & \small 4 & 
%		\small 17 & \small 68 & \small 5 \\
%		\hline
%		
%		\small{\shortstack{Standard \\ Deviation}} & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 \\
%		\hline
%		
%		\small{\shortstack{Confidence \\ Interval}} & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 & 
%		\small 180 & \small 14 & \small 97.75 \\
%		\hline
%	\end{tabular}
%	\caption{Performance comparison (in ms) of different SGX commands for \ournameplain with TPM (see Figure %\ref{fig:measurements} in appendix).}
%	\label{tab:perfcompcommand}
%\end{table*}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../usenix2019_v3.1"
%%% End: 


==> chapters/requirementAnalysis.tex <==
%!TEX root=../main.tex

%We present the extended systematization in this section.

\subsubsection{Security properties}

Security properties are broken into \emph{Strict hardware isolation} and \emph{Untrusted software dependencies}. 
\sgx uses PTT (a firmware TPM by Intel) for certain trusted computing use-cases. PTT is housed inside the CSME~\cite{intelCSME2020} and connected through DMI interface without any security around the communication channel. 
PTT uses the isolated execution environment powered by a 32-bit processor based on the Intel 486 architecture with a small dedicated SRAM (\textbf{PTT SP1: \yes}). 
CSME employs its own TCB OS with its own security ring, completely segregated from the platform security.
However, the command buffer for PTT is configured by untrusted software such as the OS (\textbf{PTT SP2: \yes}).
PTT suffers from recently found attacks CVE-2018-3659, CVE-2018-3643~\cite{csmeATTACK2018} and CVE-2019-0090, CVE-2020-0566~\cite{csmeATTACK2019} that can compromise all its use cases. As the CSME bugs are unfixable once the device is out in production, \sgx fails the objectives of strict hardware isolation (\textbf{SGX SP1:~\scros}).
Although the OS is not part of the trusted computing base of \sgx, \sgx is not OS-agnostic (\textbf{\sgx SP2:~\scros}). 
%The OS is responsible for creating and managing enclaves. 
%It allocates memory for the enclaves, manages address-translation structures for enclave memory, and copies data and code into the enclave~\cite{McKeen2016ISG}. 
%All the enclave initialization actions by the OS are securely logged by SGX and are verified on enclave launch to ensure launch-time enclave integrity. 
Intel SGX needs the OS for memory management, enclave life-cycle handling, \sgx enclaves can be interrupted by the OS, enabling an additional attack surface, \eg controlled-channel attacks~\cite{controlledsidechannel} or precise execution control of the enclave~\cite{sgxstep2017}.

In section \ref{background:tpm} we have already introduced Firmware and Hardware TPM and their features
Hardware TPM is equipped with a low-end 32-bit coprocessor and has access to a small RAM (\textbf{TPM SP1: \yes}) and NV-storage. But Firmware TPM runs on the application processor in parallel to other untrusted processes forces dependcies on insecure microarchitectural buffers  and offers no strict hardware isolation for its execution environment (\textbf{fTPM SP1: \scros}).
Software can initiate secure and encrypted session communication with the \tpm which removes the dependency on untrusted software (\textbf{TPM SP2: \yes}).

AMD-SEV runs on the processor and thus shares microarchitectural elements with untrusted software (\textbf{SEV SP1: \kinda}). 
SEV heavily depends on the hypervisor which is not part of its TCB (\textbf{SEV SP2: \scros}).
 
Google Titan~\cite{titanM} is designed and developed using a RISC-V processor combined with its own memory~\cite{titanM21} offering strict hardware isolation (\textbf{Titan SP1: \yes}). 
The goal of Titan with Android keymaster~\cite{AndroidKeystore} is to keep the key material secure with no possibility of extracting it from the hardware~\cite{AndroidKeystoreSecurityFeature}. 
The Titan backed keystore does not release keys to the system (\textbf{Titan SP2: \yes}).

TrustZone~\cite{armTZ} segments execution on the application processor into a secure world and non-secure world.
It implements restrictions on how the non-secure world interacts with the secure world. 
TrustZone also employs its own TEE OS to not depend on the rich OS (\textbf{TrustZone SP2: \scros}).
Dependencies on the external buffers also reduce the hardware isolation (\textbf{TrustZone SP1: \scros}).

Apple implements T2 the functionality with strict hardware isolation (\textbf{T2 SP1: \yes}). 
T2 requires no involvement of any untrusted software (\textbf{T2 SP2: \scros}). 

According to Microsoft, Pluton is fully compliant with the TCG TPM 2.0~\cite{TPM2Arch} specification. 
It uses a dedicated ARM M4 processor with \SI{128}{\kilo\byte} of \textit{Tightly Coupled Memory} (TCM) and \SI{64}{\kilo\byte} bootloader ROM \cite{AzureSphere}.
This configuration can provide an isolated hardware execution environment (\textbf{Pluton SP1: \yes}).
It is also unknown how the Pluton device is exposed to the platform (\eg as MMIO device) or if any untrusted software dependency is required (\eg preparing the command buffer) to perform actions on Pluton (\textbf{Pluton SP2: \unknown}).

 \begin{table}
	\centering
	\setlength{\extrarowheight}{0pt}
	\addtolength{\extrarowheight}{\aboverulesep}
	\addtolength{\extrarowheight}{\belowrulesep}
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\arrayrulecolor{black}
	\adjustbox{max width=\hsize}{
		\begin{tabular}{llllllla|alll}
			\multicolumn{1}{c}{\multirow{2}{*}{}} &
			\multicolumn{7}{c}{\begin{turn}{0}\textbf{Coprocessors}\end{turn}} &
			\multicolumn{3}{c}{\begin{turn}{0}\textbf{TEEs}\end{turn}} & \\
			\multicolumn{1}{c}{\textbf{Objectives}} &
			\multicolumn{1}{c}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}AMD~PSP\end{turn}} & \multicolumn{1}{c}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}Intel PTT in Intel CSME \quad\end{turn}} & \multicolumn{1}{c}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}Google Titan Chip ~~\end{turn}} & \multicolumn{1}{c}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}Apple T2\end{turn}} &
			\multicolumn{1}{c}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}Microsoft Pluton\end{turn}} & \multicolumn{1}{c}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}Firmware TPM\end{turn}} & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}\begin{turn}{90}Hardware TPM\end{turn}} &
			\multicolumn{1}{c}{\begin{turn}{90}Intel SGX\end{turn}} &
			\multicolumn{1}{c}{\begin{turn}{90}AMD SEV\end{turn}} &
			\multicolumn{1}{c}{\begin{turn}{90}ARM TrustZone\end{turn}} &
			\multicolumn{1}{c}{\begin{turn}{90}Keystone~RISC-V\end{turn}} \\ 
			\hline
			
			\textbf{SP. Security Properties}~ ~ & \multicolumn{1}{c}{} &  &  &  &  &  &  &  &  &  &  \\
			~ ~+ SP1.~ ~~Strict hardware isolation & \yes & \yes & \yes & \yes & \yes & \scros & \yes & \scros & \scros & \scros & \scros \\
			~ ~+ SP2.~ ~~Untrusted software dependency & \yes & \yes & \yes & \scros & \unknown & \scros & \yes & \scros & \scros & \scros & \kinda \\
			\hline
			
			\textbf{SSC. Secure Storage Capability}~ ~ & \multicolumn{1}{c}{} &  &  &  &  &  &  &  &  &  &  \\
			~ ~+ SSC1.~~Confidentiality and Integrity of storage & \scros & \scros & \yes & \kinda & \kinda & \yes & \yes & \scros & \scros & \kinda & \scros \\
			~ ~+ SSC2.~~Secure counter / Rollback protection & \scros & \scros & \kinda & \kinda & \kinda & \yes & \yes & \kinda & \kinda & \scros & \scros \\
			\hline
			
%			\textbf{TCB. Trusted Computing Building Block}~ ~ & \multicolumn{1}{c}{} &  &  &  &  &  &  &  &  &  & \\
%			~ ~+ TCB1. ~Flexible policies & \unknown & \scros & \kinda & \scros & \yes & \yes & \yes & \kinda & \scros & \scros & \scros \\
%			~ ~+ TCB2. ~Secure clock & \scros & \kinda & \scros & \scros & \kinda & \scros & \yes & \scros & \scros & \scros & \scros \\
			\hline \\	
		\end{tabular}
	}
	\caption{Comparison of Security Coprocessors and Trusted execution environments (TEEs) against objectives.}
	\label{tab:systematizationObjectives}
\end{table}

\subsubsection{Secure Storage }
 
In \sgx, support for counters depends on the Platform Service Enclave and Intel ME, which often are not available in \sgx production deployments, and already deprecated~\cite{intelCounter} (\textbf{\sgx SSC2: \kinda}). 
Moreover, these counters can be simply reset by reinstalling the SGX platform software~\cite{MateticAKDSGJC17}. 
As \sgx stores counters inside the BIOS flash storage, they do not persist across system resets~\cite{MateticAKDSGJC17} (\textbf{\sgx SSC1:\scros}).

The NV-storage implemented inside the TPM chip offers complete confidentiality and integrity of storage of secrets (\textbf{TPM SSC1: \yes}).
The aforementioned storage can be used to implement secure counters which also can provide protection against version rollback attacks for both system and third party software, and hardware (\textbf{TPM SSC2: \yes}).

AMD PSP does not employ any kind of non-volatile storage that can be used to store cryptographic secrets.
The SEV firmware is responsible for guaranteeing the confidentiality and integrity of secrets (\textbf{PSP SSC1: \scros}). 
PSP does not provide any kind of rollback protection (\textbf{PSP SSC2: \scros}). 
 
SEV SNP, \ie SEV with the secure nested paging extion, provides protection against firmware rollback but shows no evidence providing protection against virtual machine state roll back attack as it provides no secure storage capability (\textbf{SEV SSC2: \kinda} and \textbf{SEV SSC1: \scros}). 

%User secrets protected by Intel PTT are compromised (\textbf{PTT SSC1: \scros}) and Intel recommended to use \htpm instead or PTT. 
%These CVEs remove trust from Intel Dynamic Allocation Loader (DAL) and thus also the secure counter and rollback protection (\textbf{PTT SSC2: \scros}). 

Titan provides secure storage for the keys it generates or imports for its client (\textbf{Titan SSC1: \yes}). 
This storage can be used to store secure counter for rollback protection too. 
However, we are unaware of existence of such counters (\textbf{Titan SSC2: \kinda}). 

TrustZone does not offer any secure storage facility. 
Manufacturer, \eg Microsoft, implement RPMB-based storage to store counters and fuses for other secrets such as device specific OEM keys. 
However, this storage is only available to system software (\textbf{TrustZone SSC1: \kinda}). 
Additionally, TrustZone does not offer secure counter or rollback protection~\cite{armTZrollback} for the platform or software (\textbf{TrustZone SSC2: \scros}).

The T2 chip supports a very limited numbers of usecases and offers no support for non-Apple entities (\textbf{T2 VC: \scros}).
Hence, while the confidentiality and integrity of the T2 storage is available, third party code in the TEE cannot utilize it (\textbf{T2 SSC1: \yes}). 
T2 implements secure rollback protection only to the firmware, resulting in a limited counter support and rollback protection (\textbf{T2 SSC2: \yes}).

Pluton does not offer any secure storage facility other than programmable fuses to store platform specific cryptographic secrets (\textbf{Pluton SSC1: \kinda}). 
These fuses can be used to store counters to provide rollback protection. 
However, it is doubtful how much this protection can be extended beyond the platform (\textbf{Pluton SSC2: \kinda}).

%The fTPM in general does not employ any secure storage.
%Microsoft fTPM implements a secure storage through a combination of encryption with fused keys, device UUID, and Replay Protected Memory Block (RPMB) with authenticated writes and write counters. 
%We believe that this approach can be implemented (only by the manufacturer) with general fTPM (\textbf{fTPM SSC1: \yes}), which is also used to provide secure counter and rollback protection to client (\textbf{fTPM SSC2: \yes}).

Keystone hints that it can support sealed storage, trusted timers, and rollback protection.
However, it is unclear if Keystone really provides these functionalities~\cite{keystoneGithub} (\textbf{Keystone SSC1, SSC2, TCB2: \scros}). 

%\subsubsection{Trusted Computing Building Block}
%
%A desirable objective is support for flexible access-control policies for secure storage. 
%\sgx allows enclaves to implement custom authorization logic and use the result as input to the key derivation with \lstinline{EGETKEY}, making the key \emph{generation} similarly flexible as using \tpm EAP but relying on correct implementation by the enclave developers (\textbf{\sgx TCB1: \kinda}).
%Intel \sgx is not equipped with a secure source of clock but receives the clock information from the system clock, which can be modified by the untrusted OS. 
%Moreover, the OS can distort an enclave's perception of time through interrupts~\cite{Huang2021aion} (\textbf{\sgx TCB2:\scros}).
%
%TPM employes both EAP and Locality to provide access control for both access request from same security ring (\textbf{TPM HC: \yes}) and requests across security rings (\textbf{TPM VC: \yes}) respectively. 
%These access-control policies are very flexible and can be implemented from hardware, OS, to third-party software.
%They take advantage of the TPM to secure their secrets or offload their secure execution away from application processor (\textbf{TPM TCB1: \yes}). 
%TPM also implements its own secure source of clock (available at 33 MHz granularity) that makes it independent of untrusted system clock for temporal attestation and commands (\textbf{TPM TCB2: \yes}). 
%TPM also implements its own secure source of clock (available at 33 MHz granularity) that makes it independent of untrusted system clock for temporal attestation and commands (\textbf{TPM TCB2: \yes}). 
%
%To our knowledge, PSP does not provide any source of secure clock but uses the base board clock if required (\textbf{PSP TCB2: \scros}). 
%We are unable to find any available command or API that offers any types of flexible access control policies (\textbf{PSP TCB1: \unknown}).
%
%SEV depends on the mainboard clock as there is no other clock source available (\textbf{SEV TCB2: \scros}). 
%SEV provides a limited list of APIs to the VM and does not offer much flexibility around this APIs (\textbf{SEV TCB1: \scros}).
%
%PTT does not offer any service to its client (\eg OS or Hardware) that requires a clock (\textbf{PTT TCB2: \kinda}).
%PTT's use cases are limited to the OS and hardware around measured boot, platform attestation and disk encryption.
%PTT does not offer support to ring 3 software including \sgx enclaves. 
%Hence, it does not require to offer flexible policies similar to \sgx \texttt{EGETKEY} or TPM EAP (\textbf{PTT TCB1: \scros}). 
%
%To access a key, a client must provide the password related to the key. 
%This protects the access control to the key and key material but lacks flexibility (\eg flexibility offered by TPM EAP) (\textbf{Titan TCB1: \kinda}). 
%Moreover, Titan provides no secure clock service to its client (\textbf{Titan TCB2: \scros}).
%
%TrustZone does not implement any separate secure clock but uses the mainboard clock that is shared with other untrusted software (\textbf{TrustZone TCB2: \scros}).
%TrustZone allows manufacturers to implement trustlets that can run inside the TrustZone.
%Application from the rich OS can communicate through the standardized gateway communication APIs. 
%TrustZone does not add any special flexibility on the access policies to the trustlets (\textbf{TrustZone TCB1: \scros}). 
%
%Apple T2 does not offer any secure clock mechanism to the platform (\textbf{T2 TCB2: \scros}).
%Furthermore, it does not offer any support to third party code for flexible policies on command and response (\textbf{T2 TCB1: \scros}).
%
%As Pluton is fully compliant with a TPM 2.0 device, we believe it is feasible to equip Pluton with both Locality and EAP to support vertical access control (\textbf{Pluton VC: \yes}) and horizontal access control (\textbf{Pluton HC: \yes}). 
%With Locality and EAP implemented, it Pluton can also provide flexible policies (\textbf{Pluton TCB1: \yes}).
%
%The Pluton processor does not have a dedicated clock but receives clock frequency from the processor clock (the processor MT3620 is equipped with a \SI{36}{\kilo\hertz} real-time clock). 
%However, it is unclear if this clock can be manipulated by untrusted software (\textbf{Pluton TCB2: \kinda}). 
%
%An implementation of locality and EAP helps an fTPM to provide flexible policies to the client (\textbf{fTPM TCB1: \yes}).
%Due to absence of isolated hardware, an fTPM implementation always depends on the system clock (\textbf{fTPM TCB2: \scros}). 
%
%Keystone hints that it can support sealed storage, trusted timers, and rollback protection.
%However, it is unclear if Keystone really provides these functionalities~\cite{keystoneGithub} (\textbf{Keystone SSC1, SSC2, TCB2: \scros}). 
%It is also unclear to what extent Keystone provides flexibility with its policies to enclave developers (\textbf{Keystone TCB1: \scros}). 
%
%\noindent
%\linebreak
%\textbf{A.0.1 Intel SGX with Intel PTT.} Micro-architectural attacks 
%
%\noindent
%\linebreak
%\textbf{A.0.2 AMD SEV with AMD PSP.}
%
%\noindent
%\linebreak
%\textbf{A.0.3 ARM Trustzone with Google Titan.}
%
%\noindent
%\linebreak
%\textbf{A.0.4 Apple T2.}
%
%\noindent
%\linebreak
%\textbf{A.0.5. Microsoft Pluton.}
%
%\noindent
%\linebreak
%\textbf{A.0.6 Hardware and Firmware TPM.}
%
%\noindent
%\linebreak
%\textbf{A.0.7 Keystone RISC-V.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:


==> chapters/sgxAttestation.tex <==
%!TEX root=../usenix2019_v3.1.tex

%\section{\ournameplain: Enclave life-cycle handling}

%\subsection{TPM-based enclave building flow}
%\label{tpmbasedenclavebuildingflows}
%
%In \ournameplain, we moved the creation and verification of \lstinline{MRSIGNER} and \lstinline{MRENCLAVE} to \tpm by integrating the \tpm into the \sgx operations, such as \lstinline{EADD}. During enclave building, \sgx will request \tpm to create a hash of the public key of the enclave signer (\circledb{1}). This hash by the \tpm (\circledb{2}) is the \lstinline{MRSIGNER} value. Next, \sgx computes the \lstinline{MRENCLAVE} value. In step \circledb{3}, \sgx starts a hash sequence in the \tpm with \lstinline{TPM_HashSequenceStart} and will receive a sequence handle as output from \tpm (\circledb{4}). Using this handle, \sgx updates the hash digest in the \tpm with every enclave page loaded into EPC (\circledbs{5.1} \dots \circledbs{5.n}) using the \lstinline{TPM_SequenceUpdate} command. After adding the last enclave page (\circledbs{5.n}), \sgx issues \lstinline{TPM_SequenceComplete} to instruct \tpm to finalize building the hash digest (\circledb{6}). At this point, \tpm returns the hash of the measured enclave pages (\circledb{7}). This hash will be considered as the \lstinline{MRENCLAVE} value. Finally, \sgx verifies the measurement of the enclave code with the signed reference value by the enclave creator using the creator's public key (\circledb{8} \& \circledb{9}). If these steps succeed, then the enclave building is successful, otherwise it will be noted as a failed enclave building.

%\subsection{TPM-based enclave launch flow}
%\label{tpmbasedenclavelaunchflows}
%
%In \ournameplain, we inter-twine the launch control with the \tpm key creation. Figure~\ref{fig:usecaseenclacveverification} depicts the prototypical implementation of enclave launch with \tpm. The launch process in \ournameplain starts when \lstinline{EINIT} requests an enclave initialization (\circledb{A}) from LE. LE issues an LK request to \tpm as \lstinline{TPM2_Create} command (\circledb{B}) instead of the \lstinline{EGETKEY} in default \sgx. In addition, LE passes on the related enclave information to \tpm (like \lstinline{MRENCLAVE, MRSIGNER, ISVPORDID, ISVSVN}). \tpm creates an AES key and loads it in one of the key slots. We need the \tpm to generate a symmetric key to follow vanilla \sgx design and hence require a TPM2.0, which supports algorithm agility in contrast to a TPM1.2. We could employ asymmetric key cryptography with minimal changes, but for simplicity and keeping similarity with vanilla \sgx, we stuck with symmetric \tpm keys. \sgx also resets some of the \tpm PCRs and extends the enclave information received from LE into those PCRs. While there are alternative options to include the enclave information into the \tpm-based launch (e.g., via NVM or EAP), we used a PCR extension, since it not only is the simplest mechanism (e.g., no extra commands to use NVM) but also a well-known procedure from, e.g., Flicker~\cite{McCune2008}, other solutions for proof-of-execution, and measured boot mechanisms. At this point, after \tpm returned a key handle to LE, LE issues \lstinline{EINITTOKEN} generation request wrapped in an EAP session using the enclave identity information as policy digest (\circledb{C}), i.e., only if the right enclave information were extended into the PCRs the authorization succeeds. \tpm creates the \lstinline{EINITTOKEN}---HMAC of the enclave identity information---using the launch key loaded into the \tpm. \lstinline{EINITTOKEN} is returned to \lstinline{EINIT} (\circledb{D}) from LE. After \lstinline{EINIT} received the \lstinline{EINITTOKEN} it sends the token to \tpm for verification. This steps goes through LE as LE works as the single point of access to \tpm (\circledb{F}). After a successful verification, \tpm returns an acknowledgment of success to \lstinline{EINIT} (\circledb{G}) to proceed further to set the enclave's \lstinline{INIT} attribute to true. This enables a ring~3 application to execute the enclave's code using \sgx instructions. The PCRs used for the whole mechanism are reset to a predefined values for the launch of another enclave. The used PCRs are allowed to be reset, however, only by code at locality~4.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:


==> chapters/sgxLifeCycle.tex <==
%!TEX root=../ccs-template.tex

% \input{chapters/systematizationTable_multipleTEE}

% \begin{figure*}[ht]
% 	\centering
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\includegraphics[width=\textwidth]{figures/CompSignEnclave}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\includegraphics[width=\textwidth]{figures/CompgetTime}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\includegraphics[width=\textwidth]{figures/CompgetKey}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\includegraphics[width=\textwidth]{figures/CompgetReadCounter}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\includegraphics[width=\textwidth]{figures/CompQuote}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\includegraphics[width=\textwidth]{figures/CompLoadKey}
% 	\end{subfigure}
% 	\caption{QEMU overhead added (in \textit{ms}) to different SGX operations. Left columns denote end-to-end time required (on average) for each command and right columns denote the QEMU overhead added to that command (on average).}
% 	\label{fig:qemumeasurementsComp}
% \end{figure*}


%\begin{figure}[t]
%	\centering
%        \includegraphics[width=\linewidth]{figures/measurements32_1}
%	\caption{Performance comparison (in \textit{ms}) of different SGX commands for \ournameplain with \tpm }
%	\label{fig:measurements}
%\end{figure}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{figures/buildmeasurements1}
%	\caption{Performance comparison (in \textit{ms}): enclave management of \sgx against \ournameplain }
%	\label{fig:measurements_highlevel}
%\end{figure}

%\begin{table}[t]
%	\centering
%	\footnotesize
%	\begin{tabular}{|r || c | c |}
%		\hline
%		& \textbf{Host} & \textbf{Guest}  \\
%		\hline
%		\hline
%		\textbf{\scriptsize{OS}} & \scriptsize{Ubuntu 16.04.4 64bit} & \scriptsize{Ubuntu 16.04.4 64bit} \\
%		\textbf{\scriptsize{Kernel}} & \scriptsize{5.0.0+} & \scriptsize{5.0.0+} \\
%		\textbf{\scriptsize{CPU}} & \scriptsize{Intel i7-6700} & \scriptsize{Intel i7-6700} \\
%		\textbf{\scriptsize{SGX}} & \scriptsize{kvm-sgx}, \scriptsize{qemu-sgx} & \scriptsize{SGX SDK 2.0} \\
%		\hline
%	\end{tabular}
%	\caption{Prototype system configurations}
%	\label{table:prototype}
%\end{table}

The life cycle of an enclave in \sgx consists of i)~creating the enclave, ii)~initializing the enclave, iii)~executing the enclave, and iv)~removing the enclave from the processor. 
These steps are executed by executing several \sgx micro-code instructions such as \lstinline{ECREATE} to create the enclave, \lstinline{EINIT} to initialize the enclave, \lstinline{EENTER} or \lstinline{ERESUME} to enter execution phase, \lstinline{EEXIT} to take the enclave out of execution, \lstinline{AEX} to handle interrupts during enclave execution, and \lstinline{EREMOVE} to remove the enclave and free its resources. 
The enclave page cache~(EPC) is an encrypted region inside the DRAM to store the enclave pages needed for execution. 
There are other microcode instructions to handle pages related to the enclave, which are not of relevance in this paper.
Figure~\ref{fig:sgxLifeCycle} depicts the life cycle of a standard enclave in \sgx setup.

\section{Enclave Handling}
\label{app:encvCreation}

When the OS issues the \lstinline{ECREATE} instruction, it converts an EPC page into \sgx enclave control structure~(SECS). 
SECS is a specialized structure used for enclave pages and holds information about the enclave, such as its measurement. 
Every enclave can be unambiguously identified by its SECS.
\lstinline{ECREATE} marks the \lstinline{INIT} field of SECS as false to make sure the enclave's code cannot be executed before its initialization is finished and marks the enclave as uninitialized. 
At this stage, the OS can invoke the \lstinline{EADD} instruction to load the code and data pages of the enclave into the EPC. 
Every added page is measured and all measurements together in a hash-extend chain form the enclave measurement.

\subsection{Launch of Enclave}
\label{app:encvInitialization}

After loading the code and data, to initialize the enclave, the OS needs to issue the \lstinline{EINIT} instruction. 
To issue \lstinline{EINIT}, a special token called \lstinline{EINITTOKEN} is required. 
To obtain the \lstinline{EINITTOKEN}, a special management enclave of SGX, called \textit{Launch enclave}~(LE), is invoked. 
The difference between LE and a user-level enclave is that i)~LE is signed by a special Intel key hardcoded inside \sgx's implementation and ii)~\lstinline{EINIT} of LE does not require an \lstinline{EINITTOKEN} to launch the LE.

\subsubsection{\sgx Launch Control}
\label{app:sgxLaunchControl}

Upon issuing \lstinline{EINIT}, every user-level enclave has to go through an approval step using LE. 
This allows the LE to maintain control over which enclaves are allowed to launch. 
Upon a successful approval, the LE issues the \lstinline{EINITTOKEN} that authorizes an approved enclave to launch. 
The integrity of the \lstinline{EINITTOKEN} is protected by a MAC tag computed using a secret \lstinline{launch key} obtained from \lstinline{EGETKEY}. 
This step is necessary as \lstinline{EINITTOKEN} is handled by the untrusted OS. 
The \lstinline{EGETKEY} instruction implements a symmetric key derivation mechanism for \sgx's secret migration mechanism. 
\lstinline{EGETKEY} derives the key based on identity information in the current enclave's SECS and two secrets stored in secure hardware inside the \sgx-enabled processor. %But does not include enclave identification information like \lstinline{MRSIGNER} and \lstinline{MRENCLAVE}.

The \lstinline{EINITTOKEN} structure contains the identities of the approved enclave (\lstinline{MRSIGNER}, \lstinline{MRENCLAVE}) and enclave attributes. 
The token also includes the information for the launch key derivation.
Almost all the production implementation of the launch control process is proprietary and confidential, and it is hard to understand the exact behavior of the launch control through the QEMU-SGX~\cite{qemuSGX} and KVM-SGX~\cite{kvmSGX} implementation. 
To our best guess, the process is similar to a verified boot process.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/sgxLifecycle}
	\caption{SGX life cycle}
	\label{fig:sgxLifeCycle}
\end{figure}

When \lstinline{EINIT} successfully completes, it sets the enclave's init field in its SECS to true. 
This enables the enclave to execute with the help of \sgx instructions.
After the init field is set to true, \lstinline{EADD} instruction can no more be invoked, so the OS has to add all the pages that make up the enclave's initial state before executing the \lstinline{EINIT} instruction.

\subsection{Removal of Enclave}
\label{app:encvRemoval}

The OS uses the \sgx instruction \lstinline{EREMOVE} to deallocate all the enclave pages after the enclave finished executing. 
An enclave is completely destroyed when the EPC page holding its SECS is freed.

\section{SGX Attestation}
\label{sgxAttestation}

\sgx implements both local (i.e., between two enclaves) and remote (i.e., to a remote verifier) attestation. 
The attestation procedure works by creating measurements from enclave code and data. 
This process is similar to the process used in \tpm. 
The \sgx attestation procedure is very complex and cannot be implemented alone in the processor's microcode. 
Instead, \sgx uses an Intel-provided specialized enclave called \textit{Quoting Enclave}~(QE). 
This requires a mechanism for an enclave to communicate with QE in a secure manner. 
\sgx solves this problem by implementing a local attestation mechanism.
The \sgx instruction \lstinline{EREPORT} implements the scheme. 
In practice, any enclave can communicate with any other enclave using the \lstinline{EREPORT} instruction.

\subsection{Local Attestation}

An enclave proves its identity to any other target enclave through the \lstinline{EREPORT} instruction. 
For this, it produces an attestation report containing the cryptographically binding message supplied by the enclave with its measurement-based and certificate-based identities (\lstinline{MRENCLAVE} and \lstinline{MRSIGNER}). 
The cryptographic binding is accomplished by a MAC tag computed using a symmetric key called \textit{reporting key} shared between the target enclave and \sgx infrastructure.

The \lstinline{EGETKEY} instruction is used to generate the reporting key. 
This key derivation uses a secret embedded inside the processor and the target enclave's measurements.

\subsection{Remote Attestation}

During the manufacturing process, Intel embedds two secrets in the e-fuses of the processor package. 
These secrets are required to perform a remote attestation with the Intel provisioning service~(IPS). 
This process also requires the involvement of a special enclave called \textit{Provisiong Enclave} (PE), which is also an Intel-supplied enclave. 
The first step of the remote attestation process is to ensure that IPS is talking to a legitimate PE. 
For this, the PE invokes the \lstinline{EGETKEY} mechanism to create the provisioning key using one of the e-fused secrets. 
Upon a successful communication with the IPS using the \lstinline{MRSIGNER} and the provisioning key, further remote attestation takes place.

Then the IPS generates an \textit{attestation key} and forwards it to the PE. 
The PE then encrypts the attestation key using a provisioning seal key (derived using \lstinline{EGETKEY}) and hands its over to the OS to store it. 
Upon completion of the above process, the QE is invoked to perform enclave attestation. 
The enclave receives local-attestation reports and verifies them using the reporting key generated with the \lstinline{EGETKEY} instruction. 
The QE then receives the provisioning seal key to decrypt the attestation key. 
Lastly, the enclave replaces the MAC in the local attestation report with an \textit{attestation signature} produced with an attestation key.

%\section{Performance Evaluation Details}
%\label{performanceevaluationdetails}

%\input{chapters/evaluationResultTable%}

%To our understanding, \sgx's quoting features via quoting enclave has strong resemblance with TPM's quoting based software attestation mechanism. The only property that is absent in case of \sgx is the hardware supported isolation and a robust specification support enjoyed by \tpm.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:


==> chapters/usecases_backup.tex <==
%!TEX root=../samplepaper.tex

In this section, we present two case studies using \ourname. 
First, we demonstrate how \ourname protects the enclave life cycle by storing all long-term secrets in the \tpm (\Cref{UC:tpmbasedenclavebuilding}). 
Second, we show that mitigations against microarchitectural attacks can be made stronger by reducing the amount of data to protect and preventing the arbitrary restart of enclaves (\Cref{UC:mitigations}). 

\subsection{\ournameplain-backed Enclave Management}
\label{UC:tpmbasedenclavebuilding}

\noindent
%\linebreak
\textbf{Enclave Creation.} 
%\paragraph{Enclave Creation}
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.41\textwidth]{figures/secureEnclaveBuilding}
%	\caption{\tpm-backed \sgx-enclave creation using \ourname.}
%	\label{fig:usecaseenclavebuilding}
%\end{figure}
Figure~\ref{fig:usecaseenclacveverification}.a shows the steps for the \tpm-backed enclave creation. 
The creation is a two-step process, (i)~allocating enclave pages in EPC and adding code and data to those pages, and (ii)~measuring page contents (\lstinline{MRENCLAVE}) and verifying the measurement against a signed reference value by the enclave developer.

With \ourname, the creation and verification of \lstinline{MRSIGNER} and \lstinline{MRENCLAVE} is done by the \tpm. 
During enclave creation, \sgx asks (\circledb{1}) the \tpm to create a hash of the \lstinline{MRSIGNER} value (\circledb{2}). 
% Next, \sgx computes the \lstinline{MRENCLAVE} value. 
In step \circledb{3}, \sgx starts a hash sequence in the \tpm with \lstinline{TPM_HashSequenceStart} and receives a sequence handle from the \tpm (\circledb{4}). 
Using this handle, \sgx updates the hash digest inside the \tpm with every enclave page loaded into EPC (\circledbs{5.1} \dots \circledbs{5.n}) using the \lstinline{TPM_SequenceUpdate} command. 
After adding the last enclave page (\circledbs{5.n}), \sgx issues \lstinline{TPM_SequenceComplete} to instruct the \tpm to finalize the hash digest (\circledb{6}). 
The \tpm returns the hash of the measured enclave pages (\circledb{7}), \ie the \lstinline{MRENCLAVE}. 
Finally, \sgx verifies the measurement of the enclave code with the signed reference value by the enclave creator using the creator's public key (\circledb{8} \& \circledb{9}). 
If the values are the same, the enclave creation is successful.

\noindent
\linebreak
\textbf{Enclave Launch.} 
%\paragraph{Enclave Launch}
\label{UC:tpmBasedEnclaveVerification}
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.93\hsize]{figures/secureEnclaveVerification}
%	\caption{TPM-based enclave launch in \ourname.}
%	\label{fig:usecaseenclacveverification}
%\end{figure}

\begin{figure}%
	\centering
	\subfloat[\tpm communication from user space enclaves for \sgx operations.]{{\includegraphics[width=5cm]{figures/secureEnclaveBuilding} }}%
	\qquad
	\subfloat[\ournameplain \lstinline{EGETKEY} key derivation mechanism]{{\includegraphics[width=6cm]{figures/secureEnclaveVerification} }}%
	\caption{Enaclave related use-cases for \ournameplain}%
	\label{fig:usecaseenclacveverification}%
\end{figure}


A successfully-created enclave is launched using the \lstinline{EINIT} command. 
Vanilla \sgx employs a complex launch-control mechanism involving the LE, which requires a launch key (LK)~\cite{CostanD2016}. %To launch an enclave, the LE should verify the enclave and issue an \lstinline{EINITTOKEN} (the default workflow can be found in Appendix~\ref{sgxAttestation}). The \lstinline{EINITTOKEN} structure is message authenticated using an AES-CMAC key with 128-bit called \textit{launch key}~(LK).
By default, the LK is derived using the same key derivation used for sealing keys. 
The LK derivation process requires the call to originate from LE to a trusted runtime. 
The derived LK is transferred between the trusted runtime and LE via microarchitectural buffers.
As these buffers are a shared hardware element, transient-execution attacks such as Foreshadow~\cite{Bulck2018} or ZombieLoad~\cite{Schwarz2019} can extract the launch key from the buffer on an affected CPU. 
\ourname replaces this unprotected buffer transfer by encapsulating the key inside the \tpm and releasing it upon a successful authorization. 
We implement the launch control using \tpm (\cf Figure~\ref{fig:usecaseenclacveverification}.b).
In our proof-of-concept implementation, we use the LE for enclave launching. 
However, this process can be ported easily to Intel DCAP by porting the current launch service running in the LE in \ourname to the enclave launch process employed by the data center (e.g., a custom LE).

% In \ourname, we intertwine the launch control with the \tpm key creation.
Figure~\ref{fig:usecaseenclacveverification}.b depicts the prototypical implementation of the enclave launch with \ourname. 
The launch process starts when \lstinline{EINIT} requests an enclave initialization (\circledb{A}) from the LE. 
The LE issues an LK request to the \tpm with the \lstinline{TPM2_CreatePrimary} command (\circledb{B}). 
In addition, the related enclave information is passed to the \tpm (\ie \lstinline{MRENCLAVE},  \lstinline{MRSIGNER}, \lstinline{ISVPORDID}, \lstinline{ISVSVN}). 
The \tpm creates a key using the \lstinline{EINITTOKEN} KDM as supplied by the CPU. 
\sgx also resets \tpm PCRs and extends the enclave information into those PCRs (e.g., PCR 11-13). 
% While there are alternative options to include the enclave information into the \tpm-based launch (e.g., via NVM), we used a PCR extension, since it not only
The PCR extension is the simplest mechanism (e.g., no extra commands to use NVM).
It is a well-known procedure used in, e.g., Flicker~\cite{McCune2008}, other solutions for proof-of-execution~\cite{perez2006vtpm}, and measured boot mechanisms~\cite{intelTXT2021}.
After the \tpm returns a key handle, an \lstinline{EINITTOKEN} generation request is issued, wrapped in an EAP session using the enclave identity information as policy digest (\circledb{C}).
Hence, only if the correct enclave information were extended into the PCRs, the authorization succeeds.
The \tpm creates the \lstinline{EINITTOKEN}, an HMAC of the enclave identity information, using the launch key loaded into the \tpm. 
The \lstinline{EINITTOKEN} is returned to \lstinline{EINIT} (\circledb{D}) from the LE. 
\lstinline{EINIT} receives the \lstinline{EINITTOKEN} and sends it to the \tpm for verification (\circledb{F}). 
After verification, the \tpm returns an acknowledgment of success to \lstinline{EINIT} (\circledb{G}) to proceed, setting the enclave's \lstinline{INIT} attribute to true. 
This enables a ring~3 application to execute the enclave's code using \sgx instructions. 
The used PCRs are reset to their predefined values, which is possible as the code runs at locality~4.

%\paragraph{SGX Attestation (\cheading{FC2})}
\noindent
\linebreak
\textbf{SGX Attestation (FC2).} 
\label{sgxattestation}
% Intel SGX relies on software attestation and we explain here how attestation with the TPM can be integrated into SGX. 
While \sgx uses EPID~\cite{intelSGXRemAtt2016} attestation and \tpm employs DAA~\cite{cryptoeprint:2004:205}, it has been shown that EPID is an extended version of DAA and can be entirely modeled using DAA~\cite{Brickell2012}.

% \textbf{Default \sgx Attestation.} 
% \sgx performs two types of attestation, namely local and remote attestion.
For \sgx, attestation is implemented in the QE. 
\sgx employs local attestation to prove an enclave's identity to the QE. 
The QE uses the attestation keys provisioned to the platform to attest the platform information and the attested enclave's \lstinline{MRENCLAVE}.
% \textbf{Attestation with \tpm.} 
A \tpm naturally supports attestation using attestation keys, however, only of \tpm-internal data (e.g., PCR values or \tpm entities). % as any data supplied to the \tpm is considered untrustworthy. 

To attest enclaves with \ourname, we adapt the mechanism implemented by Intel and AMD for DRTM/Late-launch, where the platform attests with the TPM a small piece of code that the CPU measures. 
In DRTM, PCR17 of the \tpm is used for this measurement and is being attested.
PCR17 can only be reset to a well-known value at locality~4 by the CPU. 
Hence, a verifier is ensured that the attested measurement in PCR17 can only come from the CPU during DRTM. 
In \ourname, we designate PCR21 for \sgx attestation and set an EAP on this PCR that allows only locality~4 to read, extend, and reset this PCR. 
The \tpm can attest this policy to a remote verifier to ensure them about this policy.
During \sgx attestation, the microcode resets PCR21 and extends it with the measurement of the QE (i.e., \lstinline{MRENCLAVE} of the QE) and the report generated by the QE. 
A remote verifier can use the attested PCR21 value to check for a trusted QE and the proper report, \ie \lstinline{MRENCLAVE} and optionally supplied data to the report.
Simply extending the enclave \lstinline{MRENCLAVE} into a PCR and attesting this PCR is insufficient without ensuring that the \lstinline{MRENCLAVE} is correct and reported by a trusted entity.

\noindent
\linebreak
\textbf{Clock \& Counter.}
Getting trusted time for \sgx is difficult as an untrusted OS can manipulate the platform clock. To prevent this, \sgx receives clock information from the protected real-time clock timer \cite{Fatima2019} housed in CSME. 
However, to access this timer, \sgx enclaves require a secure path with the PSE (Platform Service Enclave)~\cite{intelPSE}. 
This communication happens over IPC and can be prone to IPC delaying attacks \cite{Fatima2019} and can distort the time for the enclave. \ournameplain overcomes this problem through the communication at locality 4, where the processor can establish a secure path to the TPM without the help of any system software (see \Cref{harpocrates}). 
\lstinline{TPM2_GetTime} and \lstinline{TPM2_ReadClock} return time and clock information to the enclaves through the hardware channel. 
The OS cannot manipulate or delay the communication as it happens in locality 4 (OS runtime receives locality 2). 
Similarly, the PSE-offered counter (stored in BIOS SPI storage) can be implemented using the NV storage offered by the \tpm. Enclaves can communicate to the counters through the above-explained locality-controlled path.
%Similarly, PSE-offered counter (stored in BIOS SPI storage:insecure\notem{that is not a sentence}) can be imitated by using the \tpm NV storage and communicated through the above explained locality controlled exclusive path.\notem{weird sentence}

\subsection{Impeding Microarchitectural Attacks}
\label{UC:mitigations}

SGX enclaves are a constant target for microarchitectural attacks~\cite{vanbulck2020phd,Schwarz2020How}, even though such attacks are considered out of scope by Intel.
Common to most of these attacks is that they observe or manipulate the microarchitectural state of hardware shared between the untrusted system and the enclave. 
Additionally, the strong attacker model and the property that enclaves can be started arbitrarily often makes it difficult to write side-channel-resilient code~\cite{Schwarz2020How}. 
Moreover, with transient-execution attacks such as Foreshadow~\cite{Bulck2018}, Spectre~\cite{Kocher2018}, RIDL~\cite{ridl2019}, ZombieLoad~\cite{Schwarz2019}, and architectural vulnerabilities such as \AE PIC~\cite{Borrello2022AEPIC}, attackers can leak sensitive data from internal CPU buffers and encrypted SGX memory even if the code is side-channel resilient. 

\noindent
\linebreak
\textbf{Preventing Transient-Execution Attacks.}
%\paragraph{Preventing Transient-execution Attacks}
\ourname provides the property of a hardware-isolated execution environment that avoids processing high-value credentials on shared hardware (i.e., caches or buffers) used by untrusted code.
A \tpm does not require any external data staging components outside its silicon (such as cache, memory, or any similar ephemeral buffers) for execution. 
\tpms are assumed to be resilient against other forms of microarchitectural attacks since no untrusted code can access the hardware of a \tpm. 
Further, by design, \tpm does not release any \tpm-managed secret keys to the outside but only \textit{key handles}. 
A transient-execution attack can, thus, only leak the \tpm key handles. 
They are only valuable for an attacker if the \tpm authorization allows attackers to use the referenced keys, which is prevented by \ourname's command authorization. 
However, in some instances, the \tpm needs to release secret data to the enclave (e.g., a decrypted symmetric key). 
With \ourname, data is loaded directly into CPU registers.
Until today, no successful transient-execution attack against the general-purpose registers of the CPU has been demonstrated~\cite{Canella2019A}. 
Note that Meltdown attacks have only been shown against system registers~\cite{rogueSystemRegRead2018,Canella2019A} as well as floating-point and the upper half of SIMD registers in specific scenarios~\cite{Stecklina2018,Moghimi2020medusa,Intel2020vector}. 
Hence, as long as a secret is only stored in an MPX register (\lstinline{BND0}-\lstinline{BND3}), it cannot be leaked using a transient-execution attack.  
Otherwise, Meltdown mitigations such as KPTI would also not be effective. 

\textbf{Proof-of-concept Evaluation.}
As a proof of concept, we reproduce the AES-NI encryption from ZombieLoad~\cite{Schwarz2019}. 
With \ourname, we can load the AES key from the \tpm directly into the CPU registers without requiring a memory load. 
Hence, the attack vector used by Schwarz~\etal\cite{Schwarz2019} is mitigated. 
To mitigate the remaining attack vector, the storing and loading of the \lstinline{XMM} registers in the SSA, we rely on Cloak~\cite{Gruss2017Cloak} to not leak any intermediate results from the registers to memory. 
We verify that the plain AES key is never stored in memory by inspecting the memory. 
Further, we are certain that the key is not stored in any microarchitectural element used for interacting with the memory, such as store buffer or line-fill buffer, that has a known vulnerability.
Consequently, current transient-execution attacks cannot leak the key from this application.
However, we cannot exclude the existence of unknown buffers that are on the data path in Cloak~\cite{Gruss2017Cloak} and that might become vulnerable in the future when research on the microarchitecture progresses.

\noindent
\linebreak
\textbf{Limiting Precise Execution Control \& Strengthening Countermeasures.}
%\paragraph{Limiting Precise Execution Control \& Strengthening Countermeasures}
%This class of attacks, most prominently \textit{SGX-STEP}~\cite{sgxstep2017},
Due to the strong attacker model, \sgx enclaves can be interrupted at an arbitrary point, allowing precise execution control~\cite{Schwarz2020How}. 
With SGX-step~\cite{sgxstep2017}, enclaves are interrupted after every instruction, allowing an attacker to inspect the microarchitectural state after every instruction. 
Hence, even a small side-channel leakage can be amplified~\cite{sgxstep2017}. 
Additionally, with zero stepping~\cite{Bulck2018}, an instruction can be re-executed arbitrarily often. 
The constant interruptions result in constantly storing and loading of the enclave state, resulting in more reliable transient-execution attacks~\cite{Bulck2018,Schwarz2019}. 
By design, \ourname does not store secrets stored in the MPX registers to memory in plain, preventing the leakage of these values (\cf \Cref{harpocrates}). 

While \ourname cannot directly prevent precise execution control, its persistent storage can be used to keep track of how often an enclave was interrupted. 
Enclaves can detect interrupts by either using Intel TSX~\cite{Shih2017tsgx,Gruss2017Cloak} if it is available or using the more generic technique of relying on overwritten values in the SSA~\cite{Oleksenko2018varys,Chen2019defeating}.
However, currently, enclaves cannot store the information about interrupts across enclave restarts. 
With \ourname, an enclave can track the number of interrupts across enclave restarts. 
Due to this persistent storage, an enclave can refuse to start if it suffered from an excessive number of interrupts. 

Generally, \ourname allows enclaves to keep information across restarts. 
This feature strengthens state-of-the-art countermeasures against microarchitectural attacks. 
T-SGX~\cite{Shih2017tsgx}, Varys~\cite{Oleksenko2018varys}, or D\'ej\`a Vu~\cite{Chen2017detecting} drastically reduce the observable leakage during one enclave run. 
However, as they cannot prevent an enclave from being restarted arbitrarily often, leakage is still possible~\cite{Jiang2020monitoring}.
Leveraging the secure counters from \ourname strengthens such countermeasures to prevent an enclave from starting if too many abnormal events have been observed during the execution. 

\textbf{Proof-of-concept Evaluation.}
We implemented the restart limitation into the sample enclave of T-SGX~\cite{Shih2017tsgx}. 
The enclave first increments a counter stored in the \tpm and retrieves the current value. 
This value is the number of times the enclave has been started. 
Note that it is important to increase the counter before checking it to prevent an attacker from terminating the enclave before the counter is updated. 
Only if the current counter value is below an enclave-defined threshold, the enclave continues to provision the secrets. 
Otherwise, the enclave simply aborts its execution. 
It is not even necessary to hardcode the number of executions into the enclave. 
The limit can be obtained from a remote server to gradually increase the number of allowed executions over time. 
Contrary to the number of enclave executions, it is possible to store this threshold in a sealed data blob. A rollback attack would only decrease the number of remaining enclave executions, providing no advantages to an attacker. 

As the entire check only happens once at enclave startup, this is a one-time overhead. 
With T-SGX, the time it takes to create and launch the enclave is \SI{19.66}{\milli\second}$\pm$\SI{0.016}{\milli\second} ($n$ = 1000). 
Increasing, reading, and comparing the timer with \ourname takes on average \SI{17.45}{\milli\second}$\pm$\SI{0.23}{\milli \second}.
%Hence, this is a one-time overhead of 47.02\,\%.
%There is no performance overhead when the enclave is running.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../bare_conf"
%%% End:

